Subword-Delimited Downsampling for Better Character-Level Translation

Subword-level models have been the dominant paradigm in NLP. However, character-level models have the benefit of seeing each character individually, providing the model with more detailed information that ultimately could lead to better models. Recent works have shown character-level models to be competitive with subword models, but costly in terms of time and computation. Character-level models with a downsampling component alleviate this, but at the cost of quality, particularly for machine translation. This work analyzes the problems of previous downsampling methods and introduces a novel downsampling method which is informed by subwords. This new downsampling method not only outperforms existing downsampling methods, showing that downsampling characters can be done without sacrificing quality, but also leads to promising performance compared to subword models for translation.

==> extra.tex <==
\subsection{Pooling Attention}
While downsampling methods such as GBST can reduce the length of a sequence by an integer factor, this can be limiting due to the often uneven and inconsistent ratio of characters to words in most sentences. As such, we propose a transformer-like method of downsampling from characters to words known as pooling attention.

Pooling attention is inspired by the \verb|HopfieldPooling| layer proposed in \citet{ramsauer2020hopfield}, and it is identical to the cross-attention in terms of its association of two sequences. Considering 2 sequences $X$ and $Y$ as input, standard cross-attention will output $Y'$ (which is identical in length to $Y$), where each token within is informed by a weighted sum of tokens from $X$.

Pooling attention uses this same principle to downsample a single \st{single} sequence. In pooling attention, $X$ is our initial input (i.e. our sequence of characters), and $Y$ is a static input of the desired length. For the static input, we use sinusoidal positional embeddings.\todo{What is the role of such initialisation?} Thus the resulting $Y'$ is a sequence of desired length, which each token being informed by our character sequence $X$. A visualization of pooling attention is shown in Figure \ref{fig:pool_attn}.

\begin{figure}
    \centering
    \includegraphics[scale=0.4]{pool_attn.png}
    \caption{Example of pooling attention for the input ``Hello world''. The numbers denote the position of each token, which would initially be represented with a sinusoidal embedding. The solid lines indicate the intuitive associations, dashed lines indicate non-intuitive (but potentially useful) associations, and red dashed lines indicate masked associations for causal generation.}
    \label{fig:pool_attn}
\end{figure}


As such, pooling attention allows for a sequence\todo{an output sequence?} length of any arbitrary factor. For sequences which require causal training (like the decoder for translation), a causal attention mask can simply be applied to prevent information leak.  

To boost the performance of pooling attention,\todo{so this is not the standard approach, what would that be?} we use a Transformer block similar to the original cross attention block, shown in Figure \ref{fig:pool_block}.\todo{not clear to me what this comparison aims to show} It consists of a pooling attention layer, followed by a self attention layer. We swap the ordering of the self attention due to the initial input being static sinusoidal embeddings.


\begin{figure}
    \centering
    \includegraphics[scale=0.5]{pool_attn_block.png}
    \caption{Pooling attention block (left), compared to the traditional cross attention block (right). Each module within the block also includes the standard dropout, layer normalization, and residual connections.}
    \label{fig:pool_block}
\end{figure}



\section{Adaptation from the Subword-Level to Character-Level}
Given that SDD downsamples from characters to subwords, this raises the question, can we adapt existing subword models to perform as character models? Specifically, as we see character models are more robust to character noise, can we adapt subword models to be more robust to character noise?

\begin{figure}
    \centering
    \includegraphics[scale=0.3]{downsamp.png}
    \caption{Adaptation scheme. ``\#'' indicates masked characters, in this case for the token ``\_world''. ``\_'' indicates the character added by the subword tokenizer to distinguish words.}
    \label{fig:lee_adapt}
\end{figure}

To accomplish this, we use a pretrained encoder model, Roberta, and attach the SDD to the front, as shown in Figure \ref{fig:lee_adapt}. We then freeze the encoder, and train only the downsampling module. We train it on a modified masked-language modeling (MLM), with the modifications as follows:
\begin{itemize}
    \item For a subword token that would be masked, all the characters in the subword are masked.
    \item For a subword token that would be replaced, it is replaced with a same-character-length subword token.
\end{itemize}
These two modifications make the MLM objective easier, as it gives the model information on the lengths of the missing words. However, since the majority of the model is frozen, we expect the model will not be negatively affected. 

